Analytical Aircraft State and IMU Signal Generator from Smoothed Reference Trajectory

This work presents a method for generating position, attitude, and velocity states for an aircraft following a smoothed reference trajectory. The method also generates accelerometer and gyro measurements consistent with the aircraft states. This work describes three corner smoothing algorithms for generating a smoothed reference trajectory from a series waypoints that accounts for limitations in the physical system. The smoothed reference trajectory, and curvilinear motion theory are used to generate the lower-order states. A coordinated turn maneuver is then applied to generate accelerometer and gyro measurement estimates.

==> sections/CovariancePropagation.tex <==
One way to use the generated accelerations and angular rates is to apply them to an inertial
navigation model for covariance propagation.This section presents
the general form of the nonlinear equations that define the dynamics
and covariance propagation for an inertial navigation system. The general equations follow the common derivation for the continuous-discrete extended Kalman filter \cite{beard_randy_small_2012}.

The continuous-time truth dynamics evolve based on the true state of the system, $\boldsymbol{x}\in\mathbb{R}^{n}$,
and white noise $\boldsymbol{w}\in\mathbb{R}^{n_{w}}$ with power
spectral density (PSD) $S_{w}\left(t\right)$ and is given by

\textbf{
\begin{equation}
\dot{\boldsymbol{x}}=\boldsymbol{f}\left(\boldsymbol{x},\boldsymbol{w},t\right)\label{eq:nonlin1}
\end{equation}
}An example of truth dynamics for a UAV are the rigid body rotational,
translational, and sensor dynamics.

Observations of the true state of the system are made through measurements, both in continuous-time and discrete-time. The continuous measurements, $\tilde{\boldsymbol{y}}\in\mathbb{R}^{n_{\tilde{y}}}$, can be 
used to propagate of the navigation state and are corrupted by continuous white noise, $\boldsymbol{\eta}$,
with noise strength $Q$. The continuous measurement equation is given by
\begin{equation}
\tilde{\boldsymbol{y}}=\boldsymbol{c}\left(\boldsymbol{x}\right)+\boldsymbol{\eta}\label{eq:nonlin2}
\end{equation}
Discrete measurements,
$\tilde{\boldsymbol{z}}\in\mathbb{R}^{n_{z}}$ corrupted by noise
$\boldsymbol{\nu}_{k}$ with variance $R_{\nu}$, are processed by
the Kalman filter to provide corrections to the navigation state.
\begin{equation}
\tilde{\boldsymbol{z}}_{k}=\boldsymbol{h}\left(\boldsymbol{x}_{k}\right)+\boldsymbol{\nu}_{k}\label{eq:nonlin4}
\end{equation}
Examples of continuous measurements, $\tilde{\boldsymbol{y}}$, for
a UAV include accelerometer and gyro measurements for propagating
the state. In contrast, an example of discrete measurements used to
update the navigation state is GPS position measurements.

As previously discussed, the navigation state, $\hat{\boldsymbol{x}}\in\mathbb{R}^{\hat{n}}$
is propagated using the continuous inertial measurements (commonly
referred to as ``model replacement'' \cite{lefferts_kalman_1982}), and updated via the Kalman
gain $\hat{K}_{k}$ and the residual, i.e. the difference between
the discrete measurement and the predicted discrete measurement $\hat{\tilde{\boldsymbol{z}}}\in\mathbb{R}^{n_{z}}$
\textbf{
\begin{equation}
\dot{\hat{\boldsymbol{x}}}=\hat{\boldsymbol{f}}\left(\hat{\boldsymbol{x}},\tilde{\boldsymbol{y}}\right)\label{eq:nonlin5}
\end{equation}
\begin{equation}
\hat{\boldsymbol{x}}_{k}^{+}=\hat{\boldsymbol{x}}_{k}^{-}+\hat{K}_{k}\left[\tilde{\boldsymbol{z}}_{k}-\hat{\tilde{\boldsymbol{z}}}_{k}\right]\label{eq:nonlin6}
\end{equation}
\begin{equation}
\hat{\tilde{\boldsymbol{z}}}_{k}=\hat{\boldsymbol{h}}\left(\hat{\boldsymbol{x}}_{k}\right)\label{eq:nonlin7}
\end{equation}
\begin{equation}
\hat{K}_{k}=\hat{P}_{k}^{-}\hat{H}_{k}\left(\hat{H}_{k}\hat{P}_{k}^{-}\hat{H}_{k}^{T}+\hat{R}_{\nu}\right)^{-1}\label{eq:nonlin8}
\end{equation}
}
The navigation state covariance $\hat{P}$ is similarly propagated
and updated using
\textbf{
\begin{equation}
\dot{\hat{P}}=\hat{F}\hat{P}+\hat{P}\hat{F}^{T}+\hat{B}\hat{Q}\hat{B}^{T} \label{eq:phatdot}
\end{equation}
}and\textbf{
\begin{equation}
\hat{P}_{k}^{+}=\left(I-\hat{K}_{k}\hat{H}_{k}\right)\hat{P}_{k}^{-}\left(I-\hat{K}_{k}\hat{H}_{k}\right)^{T}+\hat{K}_{k}\hat{R}_{\nu}\hat{K}_{k}^{T}\label{eq:nonlin10}
\end{equation}
}where the quantities $\hat{\boldsymbol{f}}$, $\hat{\boldsymbol{h}}$,
$\hat{F}$, $\hat{H}$, $\hat{Q}$, and $\hat{R}_{\nu}$ are all obtained
from the navigation design model.

The continuous measurements corresponding to \eqref{eq:nonlin2},
which are used to propagate the navigation state, consist of an accelerometer
and a gyro whose z axis is aligned with the local vertical, corrupted
by continuous white noise.
\begin{equation}
\underset{\tilde{\boldsymbol{y}}}{\underbrace{\left[\begin{array}{c}
\tilde{\boldsymbol{a}}^{b}\\
\tilde{\boldsymbol{\omega}}^{b}
\end{array}\right]}}=\underset{\boldsymbol{c}\left(\boldsymbol{x}\right)}{\underbrace{\left[\begin{array}{c}
\boldsymbol{a}^{b}+\boldsymbol{b}_{a}\\
\boldsymbol{\omega}^{b}+\boldsymbol{b}_{g}
\end{array}\right]}}+\underset{\text{\ensuremath{\boldsymbol{\eta}}}}{\underbrace{\left[\begin{array}{c}
\boldsymbol{n}_{a}\\
\boldsymbol{n}_{\omega}
\end{array}\right]}}\label{eq:vehicle6}
\end{equation}
The true body-frame accelerations $(\boldsymbol{a}^b)$ of the aircraft are computed by rotating the navigation frame accelerations in \eqref{eq:curvilinear_accel_final} to the body-frame with 
\begin{equation}
\boldsymbol{a}^b = \hat{R}_n^b \boldsymbol{a}^n
\end{equation}
The body-frame angular rates $(\boldsymbol{\omega}^b)$ are given in \eqref{eq:pqr-1} where
\begin{equation}
\boldsymbol{\omega}^b = \left[\begin{array}{ccc} p & q & r \end{array}\right]^\intercal
\end{equation}
The angular rates are dependent on the path segment type and aircraft maneuver. 
\begin{comment}
\begin{equation}
\boldsymbol{a}=\left[\begin{array}{c}
\theta g\cos\phi\left(\tan^{2}\phi+1\right)\\
0\\
-g\cos\phi\left(\tan^{2}\phi+1\right)
\end{array}\right]
\end{equation}
\begin{equation}
\boldsymbol{\omega}=\left[\begin{array}{c}
\dot{\phi}-\theta\frac{g}{V_{g}}\tan\phi\\
\frac{g}{V_{g}}\tan\phi\sin\phi\\
\frac{g}{V_{g}}\tan\phi\cos\phi
\end{array}\right]
\end{equation}
\end{comment}

The preceding description has provided a framework for a general navigation system. The following paragraphs will describe a specific aircraft model with a navigation state vector defined by
\begin{equation}
\hat{\boldsymbol{x}}=\left[\begin{array}{c}
\hat{\boldsymbol{p}}^{n}\\
\hat{\boldsymbol{v}}^{n}\\
q_{\hat{b}}^{n}\\
\hat{\boldsymbol{b}}_{a}\\
\hat{\boldsymbol{b}}_{g}
\end{array}\right]
\end{equation}
where the position $(\hat{\boldsymbol{p}}^{n})$, velocity $(\hat{\boldsymbol{v}}^{n})$, and orientation quaternion $(q_{\hat{b}}^{n})$ are the main vehicle states. The state vector also has two parameter states $(\hat{\boldsymbol{b}}_{a}, \hat{\boldsymbol{b}}_{g})$ that represent the accelerometer and gyro biases.

The dynamics of the navigation state vector, corresponding to 
\eqref{eq:nonlin5}, are defined as
\begin{equation}
\underset{\dot{\hat{\boldsymbol{x}}}}{\underbrace{\left[\begin{array}{c}
\dot{\hat{\boldsymbol{p}}}^{n}\\
\dot{\hat{\boldsymbol{v}}}^{n}\\
\dot{\hat{q}}_{b}^{n}\\
\dot{\hat{\boldsymbol{b}}}_{a}\\
\dot{\hat{\boldsymbol{b}}}_{g}
\end{array}\right]}}=\underset{\hat{\boldsymbol{f}}\left(\hat{\boldsymbol{x}},\tilde{\boldsymbol{y}}\right)}{\underbrace{\left[\begin{array}{c}
\hat{\boldsymbol{v}}^{n}\\
\hat{R}_{b}^{n}\left(\tilde{\boldsymbol{a}}^{b}-\hat{\boldsymbol{b}}_{a}\right)+\boldsymbol{g}^{n}\\
\frac{1}{2}\hat{q}_{b}^{n}\otimes\left[\begin{array}{c}
0\\
\tilde{\boldsymbol{\omega}}^{b}-\hat{\boldsymbol{b}}_{g}
\end{array}\right]\\
-\frac{1}{\tau_{a}}\hat{\boldsymbol{b}}_{a}\\
-\frac{1}{\tau_{g}}\hat{\boldsymbol{b}}_{g}
\end{array}\right]}}\label{eq:nav1}
\end{equation}
where the accelerometer and gyro measurements are used to propagate the state and the bias parameters are modeled as first-order Gauss-Markov (FOGM) parameters with time constants $\tau_a$ and $\tau_g$, respectively. 

The Jacobian of the navigation state dynamics is given by
\begin{equation}
\hat{F}=\left[\begin{array}{ccccc}
\boldsymbol{0} & \boldsymbol{I} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0}\\
\boldsymbol{0} & \boldsymbol{0} & \left[R_{\hat{b}}^{n}\left(\tilde{\boldsymbol{a}}^{b}-\hat{\boldsymbol{b}}_{a}\right)\right]\times & -R_{\hat{b}}^{n} & \boldsymbol{0}\\
\boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & R_{\hat{b}}^{n}\\
\boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & -\frac{1}{\tau_{a}}\boldsymbol{I} & \boldsymbol{0}\\
\boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & -\frac{1}{\tau_{g}}\boldsymbol{I}
\end{array}\right]
\end{equation}
and the Jacobian of the noise mixing matrix is given by
\begin{equation}
\hat{B}=\left[\begin{array}{cccc}
\boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0}\\
-R_{\hat{b}}^{n} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0}\\
\boldsymbol{0} & R_{\hat{b}}^{n} & \boldsymbol{0} & \boldsymbol{0}\\
\boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0}\\
\boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{I}
\end{array}\right]
\end{equation}
where $\boldsymbol{I}$ and and $\boldsymbol{0}$ represent $3x3$
identity and zero matrices, respectively.

This section describes a method for consuming the accelerations and angular rates of a smoothed reference trajectory to efficiently propagate the covariance of the navigation system. A path planner or navigation system designer can use this information in conjunction with Sections \ref{sec:Path-Smoothing} and \ref{sec:State-Generation} to determine the validity of the planned path or guide the navigation system design. This can be accomplished by creating a simulator to generate a smoothed candidate trajectory, and propagate the navigation system covariance. If desired, the simulator could also provide discrete-time measurements and the navigation system covariance can be updated according to \eqref{eq:nonlin10}.

